Variable Time-Step MPC for Agile Multi-Rotor UAV Interception of Dynamic Targets

Agile trajectory planning can improve the efficiency of multi-rotor Uncrewed Aerial Vehicles (UAVs) in scenarios with combined task-oriented and kinematic trajectory planning, such as monitoring spatio-temporal phenomena or intercepting dynamic targets. Agile planning using existing non-linear model predictive control methods is limited by the number of planning steps as it becomes increasingly computationally demanding. That reduces the prediction horizon length, leading to a decrease in solution quality. Besides, the fixed time-step length limits the utilization of the available UAV dynamics in the target neighborhood. In this paper, we propose to address these limitations by introducing variable time steps and coupling them with the prediction horizon length. A simplified point-mass motion primitive is used to leverage the differential flatness of quadrotor dynamics and the generation of feasible trajectories in the flat output space. Based on the presented evaluation results and experimentally validated deployment, the proposed method increases the solution quality by enabling planning for long flight segments but allowing tightly sampled maneuvering.

==> Makefile <==
PDFLATEX := pdflatex
BIBTEX   := bibtex

TARGET   := main

all: pdf
#	$(MAKE) -C . bib
	$(MAKE) -C . pdf
#	@echo -e "\033[0;33m"
#	$(MAKE) -C . pdf
#	@echo -e "\033[0m"

pdf: 
	$(PDFLATEX) $(TARGET)

bib:
	@echo -e "\033[0;32m"
	$(BIBTEX) $(TARGET)
	@echo -e "\033[0m"

clean c:
	$(RM) -rv $(TARGET).log $(TARGET).aux $(TARGET).toc $(TARGET).lof $(TARGET).lot $(TARGET).blg $(TARGET).bbl *.out

cleanall ca: clean
	$(RM) -rv $(TARGET).pdf $(TARGET).bbl


==> support/comrob-ds/Makefile <==
#
# Date:      2018/12/18 12:07
# Author:    Jan Faigl
#

MK_DIR=../../Mk

paper=3dmkop
EXT_DIR:=/comrob-ds/papers/manuscripts/3dmkop/fig

#DIRS=presentation

FILES=\
      35_iter_10.pdf\
      35_iter_100.pdf\
      35_iter_1029.pdf\
      35_iter_400.pdf\
      control_errors.pdf\
      cover_40.pdf\
      exact_kinematic_constraints_tsili_2_3d_40.pdf\
      hardware_expt_nine_imgs.pdf\
      interception_3d_1.pdf\
      interception_3d_2.pdf\
      interception_3d_3.pdf\
      real_world_experiment.png\
      tsili2_3d_40.pdf\
      tsili2_3d_dt_40.pdf\
      tsili_2_10_vel.pdf\
      tsili_2_15.pdf\
      tsili_2_15_dt.pdf\
      tsili_2_15_vel.pdf\
      tsili_2_20_vel.pdf\
      tsili_2_25.pdf\
      tsili_2_25_dt.pdf\
      tsili_2_25_vel.pdf\
      35_iter_10-crop.pdf\
      35_iter_100-crop.pdf\
      35_iter_1029-crop.pdf\
      35_iter_400-crop.pdf\
      control_errors-crop.pdf\
      tsili_2_10_vel-crop.pdf\
      tsili_2_15-crop.pdf\
      tsili_2_15_dt-crop.pdf\
      tsili_2_15_vel-crop.pdf\
      tsili_2_20_vel-crop.pdf\
      tsili_2_25-crop.pdf\
      tsili_2_25_dt-crop.pdf\
      tsili_2_25_vel-crop.pdf

include $(MK_DIR)/support.comrob-ds-cache.mk


